Cross-Impact of Order Flow Imbalance in Equity Markets

We investigate the impact of order flow imbalance (OFI) on price movements in equity markets in a multi-asset setting. First, we propose a systematic approach for combining OFIs at the top levels of the limit order book into an integrated OFI variable which better explains price impact, compared to the best-level OFI. We show that once the information from multiple levels is integrated into OFI, multi-asset models with cross-impact do not provide additional explanatory power for contemporaneous impact compared to a sparse model without cross-impact terms. On the other hand, we show that lagged cross-asset OFIs do improve the forecasting of future returns. We also establish that this lagged cross-impact mainly manifests at short-term horizons and decays rapidly in time.

==> tables/CI_PI_R2.tex <==
\begin{tabular}{c|r|cccc}\hline
   & & $\text{PI}$ (\%) & $\text{CI}$ (\%) & $\Delta R^2$ (\%) & $p$-Value \\\hline 
\multirow{2}{*}{$\text{ofi}^{1}$} & In-Sample  & 71.16 & {\bf 73.87} & 2.71 & 0.00 \\
& Out-Of-Sample & 64.64 & {\bf 66.03} & 1.39 & 0.00 \\\hline
\multirow{2}{*}{$\text{ofi}^{I}$} & In-Sample  & 87.14 & {\bf 87.85} & 0.71 & 0.00 \\
& Out-Of-Sample & {\bf 83.83} & 83.62 & -0.21 & 1.00 \\\hline
\end{tabular}

==> tables/CI_R2_Deep.tex <==
\begin{tabular}{c|r|cccc}\hline
   & & $\text{PI}$ (\%) & $\text{CI}$ (\%) & $\Delta R^2$ (\%) & $p$-Value \\\hline
\multirow{2}{*}{$[\text{ofi}^{1}, \dots, \text{ofi}^{10}]$} & In-Sample  & 89.28 & 89.61 & 0.33 & 0.00 \\
& Out-Of-Sample & 84.21 & 83.35 & -0.86 & 1.00 \\\hline
\end{tabular}

==> tables/Eco_Forecast_Ens.tex <==
\begin{tabular}{lcc}
    \toprule
    & ($\textbf{AR}$, $\textbf{FPI}^{[1]}$) &  ($\textbf{CAR}$, $\textbf{FCI}^{[1]}$) \\\midrule
PnL  & 0.23 & 0.46 \\
& (0.10) & (0.17) \\
\bottomrule
\end{tabular}

==> tables/Forward_Sup.tex <==
\begin{tabular}{ll|cccc|cccc|cccc}\hline
   & & \multicolumn{4}{c}{2017} & \multicolumn{4}{c}{2018} & \multicolumn{4}{c}{2019} \\\hline
   & & Q1 & Q2 & Q3 & Q4 & Q1 & Q2 & Q3 & Q4 & Q1 & Q2 & Q3 & Q4 \\\hline
\multirow{2}{*}{OOS $R^2$ (\%)}  & $\text{F-PI}^{[1]}$ & -17.59  & -16.85  & -17.27  & -17.01  & -17.08  & -17.1   & -17.83  & -17.92  & -15.9   & -17.86  & -18.91  & -18.23  \\
& $\text{F-CI}^{[1]}$ & -11.33  & -11.35  & -11.11  & -10.84  & -11.79  & -11.47  & -11.82  & -13.08  & -10.43  & -12.18  & -12.75  & -12.10   \\\hline
% \multirow{2}{*}{Accuracy (\%)}  & $\text{F-PI}^{[1]}$ & 50.32   & 50.14   & 50.45   & 43.78   & 48.31   & 50.62   & 51.97   & 51.10    & 51.01   & 50.35   & 50.46   & 52.57   \\
% & $\text{F-CI}^{[1]}$ & 56.45   & 56.05   & 56.74   & 53.99   & 55.29   & 56.69   & 57.98   & 58.89   & 58.99   & 58.09   & 59.41   & 61.02   \\\hline
\multirow{2}{*}{PnL (bps)}  & $\text{F-PI}^{[1]}$ & 0.21 & 0.18 & 0.23 & -0.59 & -0.08 & 0.30 & 0.38 & 0.44 & 0.30 & 0.21 & 0.25 & 0.46    \\
& $\text{F-CI}^{[1]}$ & 0.84 & 0.79 & 0.95 & 0.89 & 1.08 & 1.08 & 1.03 & 1.23 & 1.02 & 1.08 & 1.07 & 0.87   \\\hline
\end{tabular}

==> tables/Freq_Price_Change.tex <==
\begin{tabular}{lccccccc}
\toprule
 & Mean      & Std    & 10\%  & 25\%   & 50\%  & 75\%   & 90\%  \\
\midrule
Best Bid  & 4.95 & 3.23  &  0.98  & 2.32 & 4.61 & 6.72  &  8.99 \\
Best Ask  & 4.84  & 3.18  & 0.99  & 2.30  & 4.53 & 6.64  &  9.13 \\
\bottomrule
\end{tabular}

==> tables/PI_CI_R2_OOS_TS.tex <==
\begin{tabular}{llccccccccccc}
\toprule
& $m$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\\midrule
% $\textbf{PI}^{[m]}$ (OLS) & 66.18 & 77.61 & 81.37 & 83.09 & 84.05 & 84.70 & 85.05 & 85.24 & 85.29 &  85.27 \\
\multirow{3}{*}{Top 10\%} & $\textbf{PI}^{[m]}$ & 66.18 & 77.83 & 81.69 & 83.48 & 84.59 & 85.31 & 85.81 & 86.13 & 86.33 &  86.45 \\
% \midrule
& $\textbf{CI}^{[m]}$ & 67.98 & 78.35 & 81.87 & 83.52 & 84.46 & 85.07 & 85.43 & 85.66 & 85.77 &  85.81 \\
& $\Delta R^2$ & 1.80 & 0.52 & 0.18 & 0.04 & -0.13 & -0.24 & -0.38 & -0.47 & -0.56 & -0.64 \\\midrule

\multirow{3}{*}{Middle} & $\textbf{PI}^{[m]}$ & 66.18 & 77.83 & 81.69 & 83.48 & 84.59 & 85.31 & 85.81 & 86.13 & 86.33 &  86.45 \\
% \midrule
& $\textbf{CI}^{[m]}$ & 67.98 & 78.35 & 81.87 & 83.52 & 84.46 & 85.07 & 85.43 & 85.66 & 85.77 &  85.81 \\
& $\Delta R^2$ & 1.80 & 0.52 & 0.18 & 0.04 & -0.13 & -0.24 & -0.38 & -0.47 & -0.56 & -0.64 \\\midrule

\multirow{3}{*}{Bottom 10\%} & $\textbf{PI}^{[m]}$ & 66.18 & 77.83 & 81.69 & 83.48 & 84.59 & 85.31 & 85.81 & 86.13 & 86.33 &  86.45 \\
% \midrule
& $\textbf{CI}^{[m]}$ & 67.98 & 78.35 & 81.87 & 83.52 & 84.46 & 85.07 & 85.43 & 85.66 & 85.77 &  85.81 \\
& $\Delta R^2$ & 1.80 & 0.52 & 0.18 & 0.04 & -0.13 & -0.24 & -0.38 & -0.47 & -0.56 & -0.64 \\
\bottomrule
\end{tabular}

==> tables/PI_Multi_For.tex <==
\begin{tabular}{l|r|ccc}\hline
   & & $\text{F-PI}^{[1]}$ & $\text{F-PI}^{I}$ & $\text{F-PI}^{[10]}$ \\\hline
\multirow{2}{*}{$R^2$ (\%)} & In-Sample   & 0.24 & 0.26 & 5.68 \\
& Out-Of-Sample  & -19.07 & -17.62 & -10.42 \\\hline
\multirow{2}{*}{PnL (bps)} & Forecast-implied & 0.19 & 0.20 & 0.46 \\
& Long-Short & 0.10 & 0.12 & 0.51 \\\hline
\end{tabular}

==> tables/PI_R2_deep_int.tex <==
\begin{tabular}{l|r|cccccccccc|c}\hline
&   & $\text{PI}^{[1]}$  & $\text{PI}^{[2]}$  & $\text{PI}^{[3]}$ & $\text{PI}^{[4]}$  & $\text{PI}^{[5]}$ & $\text{PI}^{[6]}$  & $\text{PI}^{[7]}$ & $\text{PI}^{[8]}$  & $\text{PI}^{[9]}$ & $\text{PI}^{[10]}$ & $\text{PI}^{I}$ \\\hline
\multirow{3}{*}{In-Sample} & $R^2$ (\%) & 71.16  & 81.61   & 85.07  & 86.69  & 87.66  & 88.30  & 88.74  & 89.04  & 89.24   & {\bf 89.38} & 87.14 \\
& $\Delta R^2$ (\%) & &  10.45 &  3.46  & 1.62  & 0.97 &  0.64 &  0.44 &  0.30  & 0.20  &  0.14 & \\
& $p$-Value & & 0.00 &  0.00  & 0.00 &  0.00 &  0.00  & 0.00  & 0.00 &  0.00  &  0.00  &  \\\hline

\multirow{3}{*}{Out-Of-Sample} &$R^2$ (\%) & 64.64  & 75.81  & 79.47  & 81.13  & 82.05  & 82.65  & 83.01  & 83.16  & 83.15   & 83.11 & \cellcolor{blue!25}83.83\\
& $\Delta R^2$ (\%) & &  11.17 &  3.66  & 1.66 &  0.92 &  0.60 &  0.36  & 0.15  & -0.01  & -0.04  & \\
& $p$-Value & & 0.00 &  0.00  & 0.00 &  0.00 &  0.00  & 0.00  & 0.00 &  0.51  &  0.93  &  \\\hline

%$t(\beta^{[m], m}_i)$ & 23.98 & 11.95 & 7.68 & 5.82 & 4.95 & 4.39 & 3.83 & 3.24 & 2.75 & 2.40 \\
%$\beta^{[m], m}_i \neq 0$ (\%) & 99.94 & 99.51 & 97.33 & 91.36 & 83.08 & 75.45 & 68.69 & 60.80 & 51.97 & 44.38 \\\hline
\end{tabular}

==> tables/R2_Int_PI_Characteristics.tex <==
\begin{tabular}{c|lc|cccc}
     &      &    &  $[0\%, 25\%)$ & $[25\%, 50\%)$  &  $[50\%, 75\%)$ & $[75\%, 100\%]$ \\\hline

%  & \multirow{2}{*}{Mkt Cap}    & IS  &  77.48    &    88.26     &   87.54     &   \textbf{91.65} \\
            %   &              & OOS & 73.50   &     84.93    &    84.67    &    \textbf{88.49} \\
\multirow{6}{*}{$\text{ofi}^{I}$} & \multirow{2}{*}{Volume}     & IS  & 70.24   &     86.27     &   92.97    &    \textbf{96.31} \\
              &              & OOS & 65.94    &    83.37   &     90.09    &    \textbf{93.09} \\
& \multirow{2}{*}{Volatility} & IS  & \textbf{88.73}    &    87.42     &   85.82    &    83.31 \\
              &              & OOS & \textbf{85.99}    &    84.48     &   82.52   &     79.00 \\
& \multirow{2}{*}{Spread}     & IS  & \textbf{97.77}    &    93.84    &    84.16     &   70.12 \\
                 &           & OOS & \textbf{94.74}    &    91.15   &     81.42    &    65.29 \\\hline  
\end{tabular}

==> tables/R2_Integrated.tex <==
\begin{tabular}{l|c}\hline
   & $\text{PI}^{I}$   \\\hline
In-Sample $R^2$ (\%) & 87.14 \\
Out-Of-Sample $R^2$ (\%) & 83.83 \\\hline
% $t(\beta_i^{I})$ & 64.85 \\
% $\beta_i^{I} \neq 0$ (\%) & 99.99 \\\hline
\end{tabular}

==> tables/R2_PI_Characteristics.tex <==
\begin{tabular}{l|ll|cccc}\toprule
     &      &    &  $[0\%, 25\%)$ & $[25\%, 50\%)$  &  $[50\%, 75\%)$ & $[75\%, 100\%]$ \\\midrule
\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Best-level}}}
& \multirow{2}{*}{Volume}     & IS  &   57.02    &    70.87    &    77.11    &    \text{80.43}       \\
                  &          & OS &   48.87   &     64.63    &    71.72     &   \text{73.86}  \\
& \multirow{2}{*}{Volatility} & IS  &     \text{73.25}   &     72.24    &    70.81   &     67.67   \\
                &            & OS &   \text{66.98}    &    66.28    &    64.61     &   59.71 \\
& \multirow{2}{*}{Spread}     & IS  & \text{83.16}    &   77.43    &     69.61      &    54.37  \\
                &            & OS & \text{77.39} &     71.84      &    63.64      &    45.37   \\\midrule  
\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{Integrated}}} & \multirow{2}{*}{Volume}     & IS  & 70.24   &     86.27     &   92.97    &    \text{96.31} \\
              &              & OS & 65.94    &    83.37   &     90.09    &    \text{93.09} \\
& \multirow{2}{*}{Volatility} & IS  & \text{88.73}    &    87.42     &   85.82    &    83.31 \\
              &              & OS & \text{85.99}    &    84.48     &   82.52   &     79.00 \\
& \multirow{2}{*}{Spread}     & IS  & \text{97.77}    &    93.84    &    84.16     &   70.12 \\
                 &           & OS & \text{94.74}    &    91.15   &     81.42    &    65.29 \\\bottomrule  
\end{tabular}
